GaussTR: Foundation Model-Aligned Gaussian Transformer for Self-Supervised 3D Spatial Understanding

3D Semantic Occupancy Prediction is fundamental for spatial understanding, yet existing approaches face challenges in scalability and generalization due to their reliance on extensive labeled data and computationally intensive voxel-wise representations. In this paper, we introduce GaussTR, a novel Gaussian-based Transformer framework that unifies sparse 3D modeling with foundation model alignment through Gaussian representations to advance 3D spatial understanding. GaussTR predicts sparse sets of Gaussians in a feed-forward manner to represent 3D scenes. By splatting the Gaussians into 2D views and aligning the rendered features with foundation models, GaussTR facilitates self-supervised 3D representation learning and enables open-vocabulary semantic occupancy prediction without requiring explicit annotations. Empirical experiments on the Occ3D-nuScenes dataset demonstrate GaussTR's state-of-the-art zero-shot performance of 12.27 mIoU, along with a 40% reduction in training time. These results highlight the efficacy of GaussTR for scalable and holistic 3D spatial understanding, with promising implications in autonomous driving and embodied agents. The code is available at https://github.com/hustvl/GaussTR.

==> tab/2_ablat_combs.tex <==
\begin{table*}[ht]
    \centering
    \begin{minipage}[t]{0.4 \linewidth}
        \centering
        \begin{minipage}[t]{\linewidth}
            \centering
            \begin{tabular}{ c c | r r }
                \toprule
                Metric3D   & CLIP       & \multicolumn{1}{c}{IoU}            & \multicolumn{1}{c}{mIoU} \\
                \midrule
                           & \checkmark & \multicolumn{2}{c}{not convergent}                            \\
                \checkmark &            & 43.87                              & \multicolumn{1}{c}{-}    \\
                \checkmark & \checkmark & \textbf{45.19}                     & \textbf{11.70}           \\
                \bottomrule
            \end{tabular}
        
            \caption{\textbf{Ablation on geometric and semantic alignment.}}
            \label{table:ablat_geom_n_sem}
        \end{minipage}

        \begin{minipage}{\linewidth}
            \centering
            \begin{tabular}{ c c | r r }
                \toprule
                DINO       & FeatUp     & \multicolumn{1}{c}{IoU} & \multicolumn{1}{c}{mIoU} \\
                \midrule
                           &            & 42.45                   & 9.83                     \\
                \checkmark &            & 42.57                   & 10.26                    \\
                \checkmark & \checkmark & 45.08                   & 11.54                    \\
                           & \checkmark & \textbf{45.19}          & \textbf{11.70}           \\
                \bottomrule
            \end{tabular}
        
            \caption{\textbf{Ablation on local feature enhancement.}}
            \label{table:ablat_local_feats}
        \end{minipage}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.5 \linewidth}
        \centering
        \begin{tabular}{ c c | r r }
            \toprule
            \#Queries & Seg. Aug.  & \multicolumn{1}{c}{IoU} & \multicolumn{1}{c}{mIoU} \\
            \midrule
            100       &            & 42.06                   & 10.02                    \\
            200       &            & 44.25                   & 10.73                    \\
            300       &            & \textbf{44.73}          & \textbf{10.76}           \\
            400       &            & 43.91                   & 10.54                    \\
            \midrule
            100       & \checkmark & 41.84                   & 10.53                    \\
            200       & \checkmark & 44.32                   & 11.46                    \\
            300       & \checkmark & \textbf{45.19}          & \textbf{11.70}           \\
            400       & \checkmark & 44.27                   & 11.23                    \\
            \bottomrule
        \end{tabular}
    
        \caption{\textbf{Ablation on number of queries.}}
        \label{table:ablat_num_queries}
    \end{minipage}
\end{table*}


==> tab/5_ablat_number_layers.tex <==
\begin{table}[ht]
    \centering
    \begin{tabular}{ c c | r r }
        \toprule
        \#Layers & Seg. Aug.  & \multicolumn{1}{c}{IoU} & \multicolumn{1}{c}{mIoU} \\
        \midrule
        1        &            & 43.37                   & 9.35                     \\
        2        &            & 44.06                   & 10.18                    \\
        3        &            & \textbf{44.73}          & \textbf{10.76}           \\
        4        &            & 44.79                   & 10.83                    \\
        \midrule
        1        & \checkmark & 42.49                   & 10.36                    \\
        2        & \checkmark & 43.19                   & 10.89                    \\
        3        & \checkmark & \textbf{45.19}          & \textbf{11.70}           \\
        4        & \checkmark & 44.87                   & 11.66                    \\
        \bottomrule
    \end{tabular}

    \caption{\textbf{Ablation on the number of GaussTR layers.}}
    \label{table:ablat_num_layers}
\end{table}

